The chiral Hall effect in canted ferromagnets and antiferromagnets

The anomalous Hall effect has been indispensable in our understanding of numerous magnetic phenomena. This concerns both ferromagnetic materials, as well as diverse classes of antiferromagnets, where in addition to the anomalous and crystal Hall effects, the topological Hall effect in non-coplanar antiferromagnets has been a subject of intensive research in the past decades. Here, we uncover a new flavour of the anomalous Hall effect in canted spin systems. Using advanced theoretical tools we demonstrate that upon canting, the anomalous Hall effect acquires a contribution which is sensitive to the sense of imprinted vector chirality among spins. We explore the origins and basic properties of corresponding chiral Hall effect, and closely tie it to the symmetry properties of the system. Our findings suggest that the chiral Hall effect and corresponding chiral magneto-optical effects emerge as novel versatile tools in characterizing an interplay of structure and chirality in complex magnets, as well as in tracking their chiral dynamics and fluctuations.

==> supp_commands.tex <==
%====================================================
%MAKRO NAMES
%====================================================
\newcommand{\lam}{\boldsymbol{\lambda}}
\newcommand{\gfxpath}[1]{../gfx/#1}

\newcommand{\pgi}{Peter Gr\"unberg Institut and Institute for Advanced Simulation,
Forschungszentrum J\"ulich and JARA, 52425 J\"ulich, Germany}

\newcommand{\aachen}{Department of Physics, RWTH Aachen University, 52056 Aachen, Germany}

\newcommand{\mainz}{Institute of Physics, Johannes Gutenberg University Mainz, 55099 Mainz, Germany}

%====================================================
%NOTATIONS
%====================================================

%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}[theorem]
%\newtheorem{lemma}[theorem]{Lemma}
%\DeclareMathOperator*{\moyal}{\bigstar}

\newcommand{\moyal}{\bigstar}
\newcommand{\Pf}{\mathcal{P}_\mathrm{F}}
\newcommand{\pf}{P_\mathrm{F}}

\newcommand{\Algebra}{\mathbb{A}_\hbar}
\newcommand{\algebra}{\mathbb{A}_0}

\newcommand{\realdim}{d}
\newcommand{\phasespace}{\mathbb{R}^{2\realdim}}

\newcommand{\Conn}{\mathcal{A}}
\newcommand{\Curv}{\mathcal{F}}
\newcommand{\conn}{A}
\newcommand{\curv}{F}

\newcommand{\PH}{\mathbb{P}\mathcal{H}}
\newcommand{\ph}{\mathbb{P}H}

\newcommand{\qgeom}{Q}
\newcommand{\qmetric}{g}
\newcommand{\Qgeom}{\mathcal{Q}}
\newcommand{\Qmetric}{\mathrm{g}}

\newcommand{\ad}{\mathrm{ad}}

\newcommand{\cov}{\nabla}

%====================================================
%VECTORS
%====================================================

%Standard vector command
\renewcommand{\vec}[1]{\mathbf{#1}} 

%Normalized unit vector
\newcommand{\hatn}{\hat{\mathbf{n}}}

%Cartesian unit vectors
\newcommand{\xvec}{ \hat{\mathbf{e}}_x}
\newcommand{\yvec}{ \hat{\mathbf{e}}_y}
\newcommand{\zvec}{ \hat{\mathbf{e}}_z}
\newcommand{\ivec}{ \hat{\mathbf{e}}_i}

%Spherical unit vectors
\newcommand{\rvec}{ \hat{\mathbf{e}}_r}
\newcommand{\thetavec}{ \hat{\mathbf{e}}_\theta}
\newcommand{\phivec}{ \hat{\mathbf{e}}_\phi}

%Cylindrical unit vectors
\newcommand{\rhovec}{ \hat{\mathbf{e}}_\rho}
\newcommand{\varphivec}{ \hat{\mathbf{e}}_\varphi}

%Moyal diagrams
\newcommand{\diagram}[2]{\raisebox{-.0\height}{\includegraphics[scale=1]{../gfx/moy/o#1/o#1d#2.pdf}}}
\newcommand{\smalldiagram}[2]{\raisebox{-.0\height}{\includegraphics[scale=0.7]{../gfx/moy/o#1/o#1d#2.pdf}}}
\newcommand{\smallnediagram}[2]{\raisebox{-.0\height}{\includegraphics[scale=0.7]{../gfx/moy_ne/o#1/o#1d#2.pdf}}}

%Sphere
\newcommand{\sphere}{\raisebox{-.35\height}{\includegraphics[scale=0.04]{../gfx/symbols/sphere.png}}}

%====================================================
%GENERAL MATH OPERATIONS
%====================================================

%braidning
\newcommand{\braid}{\mathrm{Braid}}
\newcommand{\abraid}{\overline{\mathrm{Braid}}}

%residue
\newcommand{\Res}[1]{
\underset{#1}{\mathrm{Res}~}
}

%c numer
\newcommand{\cnumber}{c~\text{number}}

%Absolute value
\newcommand{\abs}{\mathrm{\abs}}
%Wigner transformation
\newcommand{\wigner}{\mathcal{W}}

%image space
\newcommand{\im}{\mathrm{im}}
\newcommand{\rank}{\mathrm{rank}~}

%Reduced Moyal product
\newcommand{\rstar}{\star_\mathrm{r}}

%Left-Right Partial Tensors
\newcommand{\lpartial}{\overset{\leftarrow}{\partial}}
\newcommand{\rpartial}{\overset{\rightarrow}{\partial}}
\newcommand{\lrpartials}{\overset{\leftarrow}{\boldsymbol{\partial}}\colon\!\mathrm{\reflectbox{$\overset{\leftarrow}{\boldsymbol{\partial}}$}}}
\newcommand{\rlpartials}{\overset{\rightarrow}{\boldsymbol{\partial}}\colon\!\mathrm{\reflectbox{$\overset{\rightarrow}{\boldsymbol{\partial}}$}}}

%Unitar transformation
\newcommand{\U}{\mathcal{U}}
\newcommand{\Ud}{\mathcal{U}^\dagger}

%Trace Operation
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\Tr}{\mathrm{Tr}}

%Fracture Trace Operation
\newcommand{\fraktr}{\mathfrak{Tr}}

%Diagonal matrix
\newcommand{\diag}{\mathrm{diag}}

%Sign Function
\newcommand{\sgn}{\mathrm{sgn}}

%Identity Operation
\newcommand{\id}{\mathrm{id}}

%Encircled Moyal Star Operator
\newcommand{\circdstar}{\raisebox{-.28\height}{\includegraphics[height=0.167in]{../gfx/math/circdstar.pdf}}}

%Differential d
\newcommand{\dd}{\mathrm{d}}

%Equivalent by partial integration
\newcommand{\equivpi}{\overset{\mathrm{P.I.}}{\sim}}

%Defined as /  From definition
\newcommand{\defi}{\overset{\mathrm{def}}{=}}

%Sec hyp
\newcommand{\sech}{\mathrm{sech}}

%gradient
\newcommand{\grad}{\mathrm{grad}~}

%interior product
\newcommand{\interior}{\mathrm{i}}

%====================================================
%LATTICES
%====================================================

\newcommand{\volume}{\mathcal{V}}

%====================================================
%SUSCEPTIBILITY
%====================================================

%Landau Peierls Susceptibility
\newcommand{\lp}{\chi_\mathrm{LP}}

%Orbital Magnetic Susceptibility
\newcommand{\oms}{\chi_\mathrm{oms}}

%====================================================
%ORBITAL MAGNETIZATION
%====================================================

%Orbital moment
\newcommand{\morbbf}{\mathbf{m}_\mathrm{orb}}

%Orbital magnetization (OM)
\newcommand{\ombf}{\mathbf{m}_\mathrm{om}}
\newcommand{\om}{m_\mathrm{om}}

%Topological orbital magnetization (TOM)
\newcommand{\tombf}{\mathbf{m}_\mathrm{tom}}
\newcommand{\tom}{m_\mathrm{tom}}
\newcommand{\Tom}{M_\mathrm{tom}}

%Chiral orbital magnetization (COM)
\newcommand{\combf}{\mathbf{m}_\mathrm{com}}
\newcommand{\com}{m_\mathrm{com}}
\newcommand{\Com}{M_\mathrm{com}}

\newcommand{\chiLP}{\chi_\mathrm{LP}^{\uparrow + \downarrow}}
\newcommand{\mass}{m_\mathrm{e}}

%====================================================
%GREEN'S FUNCTIONS & MATSUBARA FORMALISM
%====================================================

%normalordering
\newcommand{\norder}[1]{: #1 :}

%wick timeordering
\newcommand{\torder}{\mathcal{T}}

\newcommand{\Corder}[1]{
	\mathcal{T}_\mathrm{c}
	\left[
	#1
	\right]
}


%Keldysh space Green's function
\newcommand{\Gk}{\underline{G}}

%Retarded Green's function
\newcommand{\Gret}{G^{\mathrm{R}}}

%Advanced Green's function
\newcommand{\Gadv}{G^{\mathrm{A}}}

%Lesser Green's function
\newcommand{\Gles}{G^<}

%Causal Green's function
\newcommand{\Gcau}{G^{\mathrm{C}}}

%Matsubara energy
\newcommand{\maten}{ \xi_n}

%Matsubara frequency
\newcommand{\matfreq}{ i \omega_n}

%====================================================
%IMPORTANT KET STATES
%====================================================

\newcommand{\fockket}{\ket{\lbrace n_q\rbrace_q}}
\newcommand{\fockbra}{\ket{\lbrace n_q\rbrace_q}}

%====================================================
%PHYSICAL CONSTANTS & OPERATORS
%====================================================

%time order operator
\newcommand{\tordering}{\mathcal{T}}

%electron mass
\newcommand{\emass}{m_\mathrm{e}}

%bold pi (canonical momentum)
%\newcommand{\bpi}{\boldsymbol{\pi}}

%Vector of Pauli matrices
\newcommand{\bsigma}{\boldsymbol{\sigma}}

%Vector of Pauli matrices (alternative notation)
%\newcommand{\btau}{\boldsymbol{\tau}}

%Exchange parameter
\newcommand{\xc}{\Delta_{\mathrm{xc}}}

%Superconducting parameter
\newcommand{\superc}{\Delta_{\mathrm{sc}}}

%fermi velocity
\newcommand{\vf}{v_\mathrm{F}}

%Rashba parameter
\newcommand{\soi}{\alpha_{\mathrm{R}}}

%Vector Rashba parameter
\newcommand{\vsoi}{\boldsymbol{\alpha}_{\mathrm{R}}}

%Boltzmann constant
\newcommand{\boltzmann}{k_\mathrm{B}}
\newcommand{\kB}{\boltzmann}

%Torque operators
\newcommand{\btorque}{\mathbf{T}}
\newcommand{\torque}{T}

%Quantum Many body field  annihilation operator
\newcommand{\qfield}{\Psi}

%====================================================
%ELECTROMAGNETISM & GAUGE FIELDS
%====================================================

%Non-Abelian vector potential
\newcommand{\apotcal}{\boldsymbol{\mathcal{A}}}

%Non-Abelian field tensor
\newcommand{\ftenscal}{\mathcal{F}}

%Classical vector potential
\newcommand{\apot}{\vec{A}}

%Magnetic field
\newcommand{\bfield}{\mathbf{B}}

%Electric field
\newcommand{\efield}{\mathbf{E}}

%Magnetization

\newcommand{\magbf}{\mathbf{m}}
\newcommand{\Magbf}{\mathbf{M}}

%====================================================
%Relativity
%====================================================
\newcommand{\spacetime}{{\mathbb{R}^{1,d}}}

%====================================================
%Fourier transformation
%====================================================
\newcommand{\fourier}[1]{
	\mathcal{F}
\left[
 #1
\right]
}

%====================================================
%TEXTMODE OPERATIONS
%====================================================

\newcommand{\kspace}{$\mathbf{k}$-space}
\newcommand{\DMI}{Dzyaloshinskii-Moriya}
\newcommand{\todo}[1]{(\textcolor{red}{#1})}
\newcommand{\remark}[1]{\textcolor{blue}{#1}}
\newcommand{\new}[1]{\textcolor{blue}{#1}}
\newcommand{\proved}[1]{(\textcolor{red}{PROVED: #1})}

